BalanceBenchmark: A Survey for Multimodal Imbalance Learning

Multimodal learning has gained attention for its capacity to integrate information from different modalities. However, it is often hindered by the multimodal imbalance problem, where certain modality dominates while others remain underutilized. Although recent studies have proposed various methods to alleviate this problem, they lack comprehensive and fair comparisons. In this paper, we systematically categorize various mainstream multimodal imbalance algorithms into four groups based on the strategies they employ to mitigate imbalance. To facilitate a comprehensive evaluation of these methods, we introduce BalanceBenchmark, a benchmark including multiple widely used multidimensional datasets and evaluation metrics from three perspectives: performance, imbalance degree, and complexity. To ensure fair comparisons, we have developed a modular and extensible toolkit that standardizes the experimental workflow across different methods. Based on the experiments using BalanceBenchmark, we have identified several key insights into the characteristics and advantages of different method groups in terms of performance, balance degree and computational complexity. We expect such analysis could inspire more efficient approaches to address the imbalance problem in the future, as well as foundation models. The code of the toolkit is available at https://github.com/GeWu-Lab/BalanceBenchmark.

==> taxnomy.tex <==
\section{Taxonomy}
In this section, we present our taxonomy for addressing the multimodal imbalance problem, categorized into four main dimensions: Objective, Optimization, Training Procedures, and Data.

\subsection{Objectives}
Objective-based methods aim to refine the objectives in the multimodal training process to enhance overall model performance. For example, MMPareto treats multimodal learning objectives as multitask objectives. It improves the Pareto optimization algorithm for multimodal learning, boosting the generalization ability of the model across modalities.
